Worm-like instability of a vibrated sessile drop

We study the effects of vertical sinusoidal vibrations on a liquid droplet with a low surface tension (ethanol) deposited on a solid substrate. In a precise range of amplitudes and frequencies, the drop exhibits a dramatic worm-like shape instability with a strong symmetry breaking, comparable to the one observed by Pucci et al. (Phys. Rev. Lett., 106 (2011) 024503) on a vibrated floating lens. However, the geometry of our system is much simpler since it does not involve the oscillation and deformation of a liquid-liquid-air contact line. We show that the Faraday waves appearing on the surface of the droplet control its shape and we draw a systematic phase diagram of the instability. A simple theoretical model allows us to derive a relation between the elongation of the droplet and the amplitude of the Faraday wave, in good agreement with measurements of both quantities.

==> mesdef.tex <==
\usepackage{amssymb}
\usepackage{amsmath}
%\usepackage[T1]{fontenc}
%\usepackage[latin1]{inputenc}


\newcommand{\cc}{\c{c}}
\newcommand{\oC}{$^\circ$C\ }

\newcommand{\pa}{\partial}
\newcommand{\Rset}{{\mathbb R}}
\newcommand{\Cset}{{\mathbb C}}
\newcommand{\Nset}{{\mathbb N}}
\newcommand{\Zset}{{\mathbb Z}}
\newcommand{\Qset}{{\mathbb Q}}

\newcommand{\myref}[1]{(\ref{#1})}

\newcommand{\om}{\omega} 
\newcommand{\Om}{\Omega}
\newcommand{\de}{\delta}
\newcommand{\De}{\Delta}
\newcommand{\al}{\alpha}
\newcommand{\eps}{\varepsilon}
\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}
\newcommand{\be}{\beta}
\newcommand{\te}{\theta}
\newcommand{\Te}{\Theta}
\newcommand{\sig}{\sigma}
\newcommand{\vphi}{\varphi}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\tilde}[1]{\widetilde{#1}}
\renewcommand{\hat}[1]{\widehat{#1}}
\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}
\newcommand{\nab}{\nabla}

\newcommand{\demi}{\frac{1}{2}}

\newcommand{\sur}[2]{{\displaystyle\mathop{#1}_{#2}}}

\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\mcal}[1]{\mathcal{#1}}

\newcommand{\dpar}[3]{\left(\frac{\partial #1}{\partial #2}\right)_{#3}}
\newcommand{\puiss}[1]{$^{#1}$}

\newcommand{\dtk}{\frac{\mathrm{d}^3k}{(2\pi)^3}}

%\intvide = definir un carre vide place comme une integrale pour avoir de jolis {}
\newlength{\somme}
\settoheight{\somme}{$\displaystyle \int$}
\newlength{\sommep}
\settodepth{\sommep}{$\displaystyle \int$}
\addtolength{\somme}{\sommep}
\newcommand{\intvide}{\rule[-\sommep]{0cm}{\somme}}

%\intvidepetit = definir un carre vide place comme une integrale pour
%avoir de jolis {} en plus petit
\newlength{\sommebis}
\settoheight{\sommebis}{$\textstyle \int$}
\newlength{\sommepbis}
\settodepth{\sommepbis}{$\textstyle \int$}
\addtolength{\sommebis}{\sommepbis}
\newcommand{\intvidepetit}{\rule[-\sommepbis]{0cm}{\sommebis}}



